The Hierarchical Structure of Galactic Haloes: Generalised N-Dimensional Clustering with CluSTAR-ND

We present CluSTAR-ND, a fast hierarchical galaxy/(sub)halo finder that produces {\bf Clu}stering {\bf S}tructure via {\bf T}ransformative {\bf A}ggregation and {\bf R}ejection in {\bf N}-{\bf D}imensions. It is designed to improve upon Halo-OPTICS -- an algorithm that automatically detects and extracts significant astrophysical clusters from the 3D spatial positions of simulation particles -- by decreasing run-times, possessing the capability for metric adaptivity, and being readily applicable to data with any number of features. We directly compare these algorithms and find that not only does CluSTAR-ND produce a similarly robust clustering structure, it does so in a run-time that is at least $3$ orders of magnitude faster. In optimising CluSTAR-ND's clustering performance, we have also carefully calibrated $4$ of the $7$ CluSTAR-ND parameters which -- unless specified by the user -- will be automatically and optimally chosen based on the input data. We conclude that CluSTAR-ND is a robust astrophysical clustering algorithm that can be leveraged to find stellar satellite groups on large synthetic or observational data sets.

==> f_sampling.tex <==
\begin{figure*}
    \centering
    \includegraphics[trim={16mm 5mm 23mm 16mm}, clip, width=0.9\textwidth]{Images/f_Sampling_All_clusters.png}
    \vspace{-0.1cm}
    \caption{The average fraction of clusters that belong to various levels of the predicted hierarchy as it depends on $f_\mathrm{reject}$, $k_\mathrm{den}$, and the underlying feature subspace combination. These fractions are averaged over the synthetic galaxies for each combination. Clusters belonging to hierarchy levels at $L = 3$ or deeper are grouped together under the label $L > 2$. We see that for small values of $f_\mathrm{reject}$ the hierarchy almost always consists of a $L = 0$ cluster and some number of leaf clusters belonging to $L = 1$. Some leaf clusters are not returned for these values if their parent cluster is the root-level cluster, however these will be returned if $f_\mathrm{reject}$ is made large enough. For larger values of $f_\mathrm{reject}$ we see that the hierarchy deepens and the majority of the clusters belong to levels $L > 2$. While the hierarchy can be distinct between different $k_\mathrm{den}$ and feature subspace combinations, the above observations are always true to differing degrees (albeit what constitutes small/large may change). For good quality and predictable clustering results (see text in Sec. \ref{subsec:frejectvalues}) the value of $f_\mathrm{reject}$ should be chosen from the interval $[0.75, 0.95]$ -- from which we set $f_\mathrm{reject} = 0.85$ to be the standard choice for \clustar.}
    \label{fig:f_sampling}
    \vspace{-0.5cm}
\end{figure*}
